Learning Multi-Modal Self-Awareness Models for Autonomous Vehicles from Human Driving

This paper presents a novel approach for learning self-awareness models for autonomous vehicles. The proposed technique is based on the availability of synchronized multi-sensor dynamic data related to different maneuvering tasks performed by a human operator. It is shown that different machine learning approaches can be used to first learn single modality models using coupled Dynamic Bayesian Networks; such models are then correlated at event level to discover contextual multi-modal concepts. In the presented case, visual perception and localization are used as modalities. Cross-correlations among modalities in time is discovered from data and are described as probabilistic links connecting shared and private multi-modal DBNs at the event (discrete) level. Results are presented on experiments performed on an autonomous vehicle, highlighting potentiality of the proposed approach to allow anomaly detection and autonomous decision making based on learned self-awareness models.

==> sections/dbn_pl.tex <==
% Definition of circles

\colorlet{rectangle edge}{blue!50}
\colorlet{rectangle area}{red!20}

\tikzset{filled/.style={fill=rectangle area, draw=rectangle edge, thick},
    outline/.style={draw=rectangle edge, thick}}

\begin{figure}

\begin{tikzpicture}[->,
roundnode/.style={circle, draw=black!60, fill=green!5, very thick, minimum size=1.3cm},
imaginarynode/.style={circle, very thick, minimum size=1mm},
rectanglenode/.style={rectangle, draw=black!60, fill=blue!5, very thick, minimum size=1cm},
%node distance=2cm
]
%Nodes
\filldraw[color=red!60, fill=red!5, very thick, rounded corners=15pt](-2,-0.8) rectangle (5.5,3.2) node[rotate=-90]at (6,1.8) {\textbf{HMM}};
\draw[color=blue!60, very thick, rounded corners=15pt](-2,0.8) rectangle (5.5,-3.2) node[rotate=-90]at (6,-1) {\textbf{GANs}};
%\draw[filled](-0.7,-0.7) rectangle (3,3);
\node[roundnode]        (xk_1)                              {${\cal X}^{\cal I}_{k-1}$};
\node[roundnode]        (sk_1)                [above=of xk_1] {$C_{k-1}$};
\node[roundnode]        (zk_1)                [below=of xk_1] {${\cal I}_{k-1}$};

\node[imaginarynode]    (sk_2)       [left=of sk_1] {};
\node[imaginarynode]    (xk_2)       [left=of xk_1] {};
\node[imaginarynode]    (zk_2)       [left=of zk_1] {};

\node[roundnode]    (xk)                [right=0cm and 2cm of xk_1] {${\cal X}^{\cal I}_{k}$};
\node[roundnode]    (sk)                [above=of xk] {$C_{k}$};
\node[roundnode]    (zk)                [below=of xk] {${\cal I}_{k}$};



\node[imaginarynode]    (sk_n)       [right=of sk] {};
\node[imaginarynode]    (xk_n)       [right=of xk] {};
\node[imaginarynode]    (zk_n)       [right=of zk] {};

%\filldraw[color=red!60, fill=red!5, very thick](-0.7,-0.7) rectangle (3,3);
%Lines
\draw[dashed] (sk_2.east) -- (sk_1.west);
\draw[dashed] (xk_2.east) -- (xk_1.west);
\draw[dashed] (zk_2.east) -- (zk_1.west);

\draw[->] (sk_1.south) -- (xk_1.north);
\draw[->] (xk_1.south) -- (zk_1.north);


\draw[->] (xk_1.east) -- (xk.west) node[midway, above] (of_k) {${\cal P}^{\cal O}_k$};
\node[rectanglenode]    (ok)       [below=1.8cm and 0cm of of_k] {${\cal O}_{k-1}$};
\path (of_k) edge node {} (ok);

\draw[->] (sk_1.east) -- (sk.west)  node[midway, above] {$p(C_k|C_{k-1})$};


\draw[->] (sk.south) -- (xk.north) node[midway, right] {$p({\cal X}^{\cal I}_k|C_k)$};
\draw[->] (xk.south) -- (zk.north);% node[midway, left] {$p(Z_k|X_k)$};
%\draw[->] (sk_1.south) -- (of_k.north) node[midway, left]{};
\path (sk) edge node {} (of_k);

\draw[dashed] (sk.east) -- (sk_n.west);
\draw[dashed] (xk.east) -- (xk_n.west);
\draw[dashed] (zk.east) -- (zk_n.west);


%\draw[->] (rightsquare.south) .. controls +(down:7mm) and +(right:7mm) .. (zk.east);

\end{tikzpicture}
\caption{Proposed DBN switching models for private layer}
\label{fig:dbn_pl}
\end{figure}
